Joint moments of derivatives of characteristic polynomials

We investigate the joint moments of the 2k-th power of the characteristic polynomial of random unitary matrices with the 2h-th power of the derivative of this same polynomial. We prove that for a fixed h, the moments are given by rational functions of k, up to a well-known factor that already arises when h=0. We fully describe the denominator in those rational functions (this had already been done by Hughes experimentally), and define the numerators through various formulas, mostly sums over partitions. We also use this to formulate conjectures on joint moments of the zeta function and its derivatives, or even the same questions for the Hardy function, if we use a ``real'' version of characteristic polynomials. Our methods should easily be applicable to other similar problems, for instance with higher derivatives of characteristic polynomials. NOTE: More data is available on the author's website or attached to the LaTeX source of this arXiv submission.

==> MagmaCode <==
// This Magma program is associated to the paper
// Joint moments of derivatives of characteristic polynomials or of the Riemann zeta 
// function, by Paul-Olivier Dehaye

// It aims to show a working implementation, _not_ optimized for speed, of that paper.
// It also aims for clarity by computing objects as close as possible to the original paper.
// It is based on Equation (30).

// In short: THIS IS NOT OPTIMIZED FOR SPEED, but for simplicity


// // Example of use:
// data := [];
// AllMomentsComplexMUpTo(20,~data);   // this takes a while
// NumeratorNormedV(20,data);    // quick
// MomentComplexM(15,data);      // quick again
// AllMomentsComplexMUpTo(22,~data);   // this takes less time, because it's reusing everything done before
// NumeratorNormedV(22,data);    //quick again
 

K<k> := FunctionField(Rationals());

U<u> := PolynomialRing(Rationals());
// The field over which all of the numerators will be returned

m := hom<K->U|u/2>;
// The map from K to U. Remember u == 2*k

FrobeniusCoordinates := function(p1)
// Computes the Frobenius coordinates of the partition p1
// For instance, 
// > FrobeniusCoordinates([4,3,1]);
// <[ 3, 1 ], [ 2, 0 ]>
// > FrobeniusCoordinates(ConjugatePartition([4,3,1]));
// <[ 2, 0 ], [ 3, 1 ]>

     index := 1;
     while ((index le #p1) and (p1[index] ge index)) do index +:=1;end while;
     d := index-1;
     p2 := ConjugatePartition(p1);
     return <[p1[i]-i: i in [1..d]],[p2[i]-i: i in [1..d]]>;
end function;

DeterminantalPart := function(lambda)
// Computes the main determinant in each summand, associated with the partition lambda,
// given with Frobenius coordinates s,t of length d
    s := lambda[1];
    t := lambda[2];
    d := #s;
    M := Matrix(d,d,&cat[ [1 /Factorial(s[i])/Factorial(t[j])/(1+s[i]+t[j]) : j in [1..d]] : i in [1..d]]);
    return Determinant(M);
end function;

GammaPart := function(lambda)
// Computes the product of Gamma function part, as a function of the variable k defined above
// This could be optimized: since we know where poles and zeroes are initially potentially located, we could
// first figure its divisor, a matter of adding simple vectors based on the $\alpha_a(r)$ functions. 
// Then, we could see how far off from the common denominator (the $Q_r(u)$) this is, and multiply 
// by the appropriate polynomial. The interest of doing so is that the arithmetic would take place over a
// polynomial ring and not a function field. 
// We prefer to go for simplicity...
    s := lambda[1];
    t := lambda[2];
    d := #s;
    tmp := 1;
    for i := 1 to d do
        tmp *:= &*[ k+z: z in [-t[i]..s[i] ]];
    end for;
    for i := 1 to d do
        tmp /:= &*[ 2*k+z: z in [-t[i]..s[i] ]];
    end for;
    return tmp;
end function;

ComputeMomentComplexM := function(r)
// This returns (M)_r(2k) / M_0(2k) * i^r as a rational function of k,
//  i.e. the unsigned, real version without the G(k+1)^2/G(2k+1) factor
   print "Computing...",r;
   if r eq 0 then 
       return 1; 
   end if;
   partitions := Partitions(r);
   frobPartitions := [FrobeniusCoordinates(partition): partition in partitions];

   tmp := 0;
   for frobPartition in frobPartitions do
       tmp +:= DeterminantalPart(frobPartition)^2 * GammaPart(frobPartition);
   end for;
   return Factorial(r)*tmp;

//    BAD IDEA:
//    return Factorial(r)* &+[DeterminantalPart(frobPartition)^2 * GammaPart(frobPartition): frobPartition in frobPartitions];
//    bad idea because Magma has to save a huge sequence of nasty rational functions, before summing it up.
end function;

AllMomentsComplexMUpTo := procedure(R,~allMoments) 
// This computes all the moments (M)_r(u) up to r = R, starting at r=0
// and assigns it to the variable allMoments
   current := #allMoments-1; 
   if current lt R then 
      allMoments cat:= [ComputeMomentComplexM(r): r in [current+1..R]];
   end if;
end procedure;

function OddError(r)
// for the cases where we assume r = 2*h
    if IsOdd(r) then
        print "We can only compute even moments";
        assert false;
    end if;
    return r div 2;
end function;

procedure TestEnoughData(r,allMoments)
// We need to have computed the first (M)_i(2k) for i in [0..r] to be able to compute |M|_j(2k) or |V|_j(2k) for j <= r
   if r+1 gt #allMoments then
       print "We need to compute more complex moments first";
       print "You have given the first ",#allMoments, "moments (M)_i (2k), for i between 0 and ",#allMoments-1,". I need more complex moments though, please run AllMomentsComplexMUpTo more";
       assert false; 
   end if;
end procedure;


MomentComplexM := function(r,allMoments)
// Returns  (M)_r(2k) / (M)_0(2k)  as a rational function of k
// without the G(k+1)^2/G(2k+1) factor or the power of i in front
// this assumes that allMoments is long enough...
    TestEnoughData(r,allMoments);
    return allMoments[r+1];
end function;



MomentNormedM := function(r,allMoments)
// Returns  |M|_r(2k) / |M|_0(2k) as a rational function of k
// i.e. the moments without the G(k+1)^2/G(2k+1) factor
// this assumes that allMoments is long enough...
    h := OddError(r);
    TestEnoughData(r,allMoments);
    return (-1)^h * &+[Binomial(h,j) *(-1)^j* allMoments[2*h-j+1]: j in [0..h]];
end function;


// The following two functions provide the same output, but would give different analytic
// continuations if extended beyond their range of validity
MomentNormedV2 := function(r,allMoments) 
// Returns  |V|_r(2k) / |V|_0(2k) as a rational function of k
// i.e. the moments without the G(k+1)^2/G(2k+1) factor
    h := OddError(r);
    TestEnoughData(r,allMoments);
    return (-1)^h * &+[Binomial(2*h,j) *(-1/2)^j* allMoments[2*h-j+1]: j in [0..2*h]];
end function;

MomentNormedV := function(r,allMoments)
// Returns  |V|_r(2k) / |V|_0(2k) as a rational function of k
// i.e. the moments without the G(k+1)^2/G(2k+1) factor
    h := OddError(r);
    return (-1/4)^h * &+[(-4)^j * Binomial(h,j) * MomentNormedM(2*j,allMoments):j in [0..h]];
end function;

alpha := function(a,r)
// alpha(a,r) as in paper
    return Floor((-a+Sqrt(a^2+4*r))/2);
end function;

Y := function(r,uVar)
// Y_r(uVar) as in paper, denominator for the various moments
// see remark above at function GammaPart for potential optimization
     tmp := 1;
     for l := 1 to r-1 do
        if IsOdd(l) then 
           tmp *:= (uVar^2-l^2)^(alpha(l,r));
        end if;
     end for; 
     return tmp;
end function;

ComputeNumeratorComplexM := function(r) 
// Numerator X_r(u)
    return m(ComputeMomentComplexM(r)*Y(r,2*k)*2^r);
end function;

NumeratorComplexM := function(r,allMoments) 
// Numerator X_r(u)
    return m(MomentComplexM(r,allMoments)*Y(r,2*k)*2^r);
end function;

NumeratorNormedM := function(r,allMoments) 
// Numerator \hat{X}_r(u)
    h := OddError(r);
    return m(MomentNormedM(r,allMoments)*Y(r,2*k))*2^r;
end function;

NumeratorNormedV := function(r,allMoments)
// Numerator \tilde{X}_r(u)
    h := OddError(r);
    return m(MomentNormedV(r,allMoments)*Y(r,2*k))*2^(3*h)*Factorial(h)/Factorial(r);
end function;


==> NumeratorsNormedM <==
// Moments |M|(2k,2h) 
// \hat{X}_{2h}(u) for h in [1..30]

[
    u^2,
    u^4 - 8*u^2 - 6,
    u^8 - 33*u^6 + 198*u^4 + 74*u^2 - 360,
    u^10 - 81*u^8 + 1740*u^6 - 8284*u^4 - 7716*u^2 + 34020,
    u^14 - 170*u^12 + 9597*u^10 - 215560*u^8 + 1846928*u^6 - 4247400*u^4 - 12317076*u^2 + 42366240,
    u^18 - 291*u^16 + 30177*u^14 - 1379507*u^12 + 28177518*u^10 - 236602818*u^8 + 604630084*u^6 + 1570591476*u^4 - 10008266040*u^2 + 7829929800,
    u^22 - 484*u^20 + 90384*u^18 - 8378492*u^16 + 415889897*u^14 - 11196067680*u^12 + 157699171570*u^10 - 1023611526808*u^8 + 1699483809828*u^6 + 11589901952544*u^4 - 62361799232760*u^2 + 
        44754182272800,
    u^24 - 708*u^22 + 198590*u^20 - 28525892*u^18 + 2275085529*u^16 - 102837376096*u^14 + 2598141390568*u^12 - 34807690054560*u^10 + 213458763180152*u^8 - 261862022455104*u^6 - 
        3402805264433280*u^4 + 19256263380043200*u^2 - 11718802173078000,
    u^30 - 1054*u^28 + 460431*u^26 - 109299828*u^24 + 15577804767*u^22 - 1394331670638*u^20 + 79872695247657*u^18 - 2932723486507728*u^16 + 68022586503825552*u^14 - 962308385613255088*u^12 + 
        7682283932820069016*u^10 - 26475220331016986304*u^8 - 59889950570120914224*u^6 + 976582356673028315040*u^4 - 3441287004848413282800*u^2 + 1366282646437284576000,
    u^34 - 1415*u^32 + 840943*u^30 - 275540385*u^28 + 55049482221*u^26 - 7022476724835*u^24 + 584090828573565*u^22 - 31869278744265555*u^20 + 1134427249824868110*u^18 - 25880772100948222330*u^16
        + 365485578445889268104*u^14 - 2970099871666499086840*u^12 + 10773785732163438366432*u^10 + 24904735536575464181280*u^8 - 474478390713139651278576*u^6 + 1993984711160163968152080*u^4 - 
        1770512318771949573760800*u^2 + 214967318998766249916000,
    u^38 - 1936*u^36 + 1613378*u^34 - 763482608*u^32 + 228188569686*u^30 - 45387066830856*u^28 + 6175010063534400*u^26 - 582228619257664920*u^24 + 38153334469981588665*u^22 - 
        1727089884264194529640*u^20 + 53187303571666828626934*u^18 - 1085156443044105879812024*u^16 + 14030983110526151949780152*u^14 - 104970568378574512735894272*u^12 + 
        314860428693134831363109264*u^10 + 1622792626183525686630641856*u^8 - 22012387573653329226589266480*u^6 + 86838030195884447337192182400*u^4 - 51580793772130673789642484000*u^2 - 
        16096153485901786467009840000,
    u^42 - 2489*u^40 + 2696680*u^38 - 1680255016*u^36 + 670872257522*u^34 - 181264906058866*u^32 + 34169650713323772*u^30 - 4572827180326638444*u^28 + 438442537876003485825*u^26 - 
        30206665021347532836265*u^24 + 1491566078390658390507764*u^22 - 52348775880804183291920836*u^20 + 1285675848133409245540034020*u^18 - 21514517376183925985413968644*u^16 + 
        233437962040619488747137745888*u^14 - 1449822750135465453858946622304*u^12 + 2257201785416051883065319153648*u^10 + 42814237679794532693687883218064*u^8 - 
        405732551714247179963913676413120*u^6 + 1351237806156669478367283851428800*u^4 - 238016696178804880286214669096000*u^2 - 818008230134521366630270340760000,
    u^46 - 3234*u^44 + 4625889*u^42 - 3875659856*u^40 + 2124511754850*u^38 - 806769832519716*u^36 + 219369269439686974*u^34 - 43569966645681388584*u^32 + 6394966500349284793821*u^30 - 
        697603499923824195013810*u^28 + 56609963515626844161543069*u^26 - 3405564257877690519378797016*u^24 + 150683480275006035882418348016*u^22 - 4840282739789378525625033053304*u^20 + 
        110654465112040714060879771726740*u^18 - 1744865322894854155515715798513504*u^16 + 17920882568846393881179915456431376*u^14 - 102746693536956011737839946004716896*u^12 + 
        58258065903846224540915620653340464*u^10 + 4317526754086318177301604729484801920*u^8 - 37172248895427399071867509114400035200*u^6 + 112595632341199303001427494898371568000*u^4 + 
        43901445070045908419772663194617080000*u^2 - 142551920997444767577581920155048000000,
    u^50 - 3971*u^48 + 7015197*u^46 - 7303871351*u^44 + 5007974133232*u^42 - 2395263398800776*u^40 + 826432875743841142*u^38 - 209989247391810451586*u^36 + 39798373653393413572857*u^34 - 
        5667940375625784694778011*u^32 + 608600988329803214849698385*u^30 - 49269689815652401232380878579*u^28 + 2997959572660087625458690785278*u^26 - 136271425247850435893244499754674*u^24 + 
        4583405035222495967669705794192668*u^22 - 112500954690838104406415410166679124*u^20 + 1973424711351866215921013228995027208*u^18 - 23856275404774071428399928325505358264*u^16 + 
        182499972863055662899406406886091963568*u^14 - 600668354457835667944561587442749621264*u^12 - 3972074359200552046398099870276760266336*u^10 + 
        65470371749080423617887346441984967101600*u^8 - 368813285523866838374312119758071095723200*u^6 + 673369201479224265711234041622749665896000*u^4 + 
        1131568831108249854255021951481712855760000*u^2 - 1836121492022453187966033631245648414000000,
    u^58 - 5030*u^56 + 11412133*u^54 - 15500988120*u^52 + 14114988479571*u^50 - 9147546724261890*u^48 + 4373885546074871505*u^46 - 1579278567353194558620*u^44 + 437331950583901250151645*u^42 - 
        93847840407921406818157370*u^40 + 15710250265262157962152415683*u^38 - 2059256692788695156464472520560*u^36 + 211624107791707201976079423238209*u^34 - 
        17034968691550219190582141883778830*u^32 + 1070766311524164016060726705592131923*u^30 - 52275532207511767667599281640118144940*u^28 + 1966590464091001405757862509346388176870*u^26 - 
        56379140501318771578111166075800071716880*u^24 + 1212606786875975847520567258422536183993380*u^22 - 19111293958830891365048069506167671923984880*u^20 + 
        211633563947173552086164107355950284113086216*u^18 - 1481582580026543666009423576937468479736452160*u^16 + 3645636629127789420488404276917957656569937808*u^14 + 
        48289132967352170129622726296390500992890155200*u^12 - 654713015071258185392915697813400538932993477344*u^10 + 3545303792426444922969547251751413047568582862080*u^8 - 
        6464923128809593293970389875569550103491158017600*u^6 - 12604192333293440063411581661877443455690220448000*u^4 + 39456197701433725566146838211317052873294923600000*u^2 - 
        23327045852863067739147756651758136803653848000000,
    u^60 - 5990*u^58 + 16240003*u^56 - 26451986460*u^54 + 28985466320601*u^52 - 22683840056565690*u^50 + 13142833557308549955*u^48 - 5770087687027665265320*u^46 + 1949617758171939443592795*u^44 
        - 512333064272982392499222170*u^42 + 105438059100400870562633105233*u^40 - 17064727163724013043154782830940*u^38 + 2176156777184953741911575494626219*u^36 - 
        218640395436834672375914449117501350*u^34 + 17272415685819672743328341323270081113*u^32 - 1068690508972190919076113606157822167840*u^30 + 51476665405528529865951799801042910963520*u^28 -
        1914028934233660147437374922347971069051680*u^26 + 54302734992324698733350881341985431238258480*u^24 - 1156577010190546816965439189178209875571182080*u^22 + 
        18042125470008857236967623871424446842573448416*u^20 - 196991669713131146238396052148546660731983904320*u^18 + 1333023530084634557291826890323319012706319352928*u^16 - 
        2408870322730446384588255234345858380580722941440*u^14 - 58028343386741317813576935325589212920267111416064*u^12 + 717401189950313750429636030869866262084114522337280*u^10 - 
        3664271074636877397751579377565705644219535688563200*u^8 + 4757319881840240970375597003461635174064046895488000*u^6 + 24527625157156416913019610317906603847907737625440000*u^4 - 
        65617613003950377241639184272317577722251840395200000*u^2 + 39321780651471452739324818993453100035118364740000000,
    u^64 - 7303*u^62 + 24348617*u^60 - 49234933919*u^58 + 67674117965973*u^56 - 67186010684948883*u^54 + 49986479716082207709*u^52 - 28549956525117322276395*u^50 + 
        12724801237712441756448675*u^48 - 4476073664857191801168287285*u^46 + 1252245321223662545385994422923*u^44 - 280020640574733996619530542557549*u^42 + 
        50189043067204543422312224358050791*u^40 - 7216761430111632037100770585212809937*u^38 + 831864778002697219666496259413071979679*u^36 - 76683992872898809180256665164806224630329*u^34 + 
        5630724268873696148223466615165081138746432*u^32 - 327460290433688159148601346072087415660134400*u^30 + 14968740880393977519123375148770653291652197200*u^28 - 
        532522805164100973591319552255935203277049245040*u^26 + 14553645631104453226129849788662917681294504580576*u^24 - 300168764505686415080328878934915730766657271090848*u^22 + 
        4547661123525415536859139651003102370691234770386592*u^20 - 48085983700291787457868069550750978967841322967253344*u^18 + 306189884446151923183972394940433864712355742146286848*u^16 - 
        243509971156840026124581068724113544699184306868575488*u^14 - 18026112179288925665357210037974955460148983395862166016*u^12 + 
        201485487021503286558181561156616949536155711278289758720*u^10 - 942716709117924353346066491384782440401542736505247776000*u^8 + 
        529522812068382694936506504759318531843166194090496992000*u^6 + 10371659240917397830824639594676136117861577254055892320000*u^4 - 
        26653490594505924497250525536280606351570553093498500000000*u^2 + 16480728722349270562111417343312906702226445156844160000000,
    u^70 - 8633*u^68 + 34192186*u^66 - 82574606770*u^64 + 136353480261260*u^62 - 163679923078865356*u^60 + 148298555441186465808*u^58 - 103967063293264884203856*u^56 + 
        57384268920345635756487750*u^54 - 25247752339548211981803881270*u^52 + 8935365578968212850914871191748*u^50 - 2560452887250300576914855844397364*u^48 + 
        596849988999062510293868426014473788*u^46 - 113531192127838359047617228228120791100*u^44 + 17654249121036475295517669158945304166400*u^42 - 
        2245592409272682348085985903981526760793088*u^40 + 233524256815790619359553372599455217534830689*u^38 - 19821440182459591433179061370169966452183489273*u^36 + 
        1369348502550915505034276349312558634709312433490*u^34 - 76680646683299638372402283655822369357150967484330*u^32 + 3461217406543576524284404299738058433387152746780976*u^30 - 
        125008555279100484118224508812626503492042310496503728*u^28 + 3577454848592410789543955393415087935620270765211713376*u^26 - 80043782607930734057504885961589493438995894373783872480*u^24
        + 1372853452787507901132299041104890840749027813782561673440*u^22 - 17446246471612109410500090261860075929450603318463212210656*u^20 + 
        152068276017414332120876389960610400303000511890985318561728*u^18 - 671677526776381695403020803169649269169012809515321726844096*u^16 - 
        3122448564658807981462352189796911480122988303248687977872640*u^14 + 82465295695279087329610355428868598645750007233385396238112000*u^12 - 
        675511955373446070443842374548331148273050436611909707415360000*u^10 + 2299380081132110680312697378841713900812545418122916073739840000*u^8 + 
        3061668506294237622834598215932431133631099718740783375300000000*u^6 - 45779520067620064920160329012750263867407637406968368191780000000*u^4 + 
        109871230795922876357296560595267513890945272023401287392200000000*u^2 - 68475819645563460681359618868270578925210268155520326345000000000,
    u^74 - 10290*u^72 + 48891087*u^70 - 142632297644*u^68 + 286649120141778*u^66 - 422142300636675408*u^64 + 473214845197927319884*u^62 - 414146086159300805208672*u^60 + 
        288036877496780245997879910*u^58 - 161250642511677814231763965676*u^56 + 73348193517061841185171745286978*u^54 - 27296357350500383573145953930444280*u^52 + 
        8352382787315058474733260795733140616*u^50 - 2108652151271906933432381596765519788072*u^48 + 440180477053133195400868865279299131605484*u^46 - 
        76058079918392307909255166629925692499612544*u^44 + 10878412109731320265652070496161944295524152497*u^42 - 1286740731012573142559567129467047072835283041266*u^40 + 
        125635022580767555118931548048129465895242932508295*u^38 - 10096965636022006794958405140786127240328058834517308*u^36 + 665342066593714259995315689446965188723685188114006606*u^34 - 
        35766666464952736943025227812951473629537392180859226680*u^32 + 1558463998512818462495543091857694077582540452561030758672*u^30 - 
        54594608740149193907369331303523680543125409749667733358784*u^28 + 1521417809429661926114623018665725474907122602605119322431488*u^26 - 
        33249589731697043756531755980707706946190045447032776810378048*u^24 + 557899411372080513567935841383472731358376423252661724924819744*u^22 - 
        6923536740906596679384060203694805250526476548162786607002653312*u^20 + 58120122957397655040401048456457946322442651236229381329416921920*u^18 - 
        221425245239454871366786803839019146437298372947442082875388854016*u^16 - 1818639633804737172716316216289214431589242587223591819220835720960*u^14 + 
        37716401289831715579213794671244066646504051314622244979331277952000*u^12 - 287812107763851680414086242916110116630957649477169528742186394144000*u^10 + 
        809678045117892245865386382693993355927391108225485246044885382080000*u^8 + 2919991926101458314959468838824183536527800883449918537010117660000000*u^6 - 
        27257074502689698324948407405109349541638095338394039542185038960000000*u^4 + 68787406080379887463178688400248387002098288042054156826219412600000000*u^2 - 
        44383927448502493689311999114367374882622920772687196919280060000000000,
    u^78 - 11819*u^76 + 64636695*u^74 - 217512331205*u^72 + 505330728476740*u^70 - 862170768394624380*u^68 + 1122173154385925526160*u^66 - 1142853212416937812451120*u^64 + 
        927056523733126033043171550*u^62 - 606730757764937124630083769290*u^60 + 323431171613263079084977477765042*u^58 - 141424524909045863823416102209904598*u^56 + 
        50989737175125199513539021498777963220*u^54 - 15215317148829511116857421749573054305340*u^52 + 3767251316379169067508148897847211073969620*u^50 - 
        775131196041699221381744059718078245488836540*u^48 + 132617892569488603026842891923615378853067810505*u^46 - 18863176674160219214067253073131967051505049808835*u^44 + 
        2228341075335591869999708352669621589822123085961775*u^42 - 218240891189064170177771808632731053431900888618650445*u^40 + 17675494114216025947618971822852208939641135873542424288*u^38 - 
        1179839086400885947693351415470512472888794856009521237872*u^36 + 64629477604329358287752216809577827642217510291204557663300*u^34 - 
        2889885790517077071479765947004849522114853540243740812032780*u^32 + 104784082895851456062751770829734854537111862780822829969164640*u^30 - 
        3055147667939484816973507819557814585517947159120897772682882080*u^28 + 70838160044696844381501132678966846021472604018608874662277268960*u^26 - 
        1285341600078757057934654857366844563309145216076391251105258901920*u^24 + 17761622284199995660897916810162913694342394039458885683813811372800*u^22 - 
        176213628597059045220212018442528407200461007826246858384298116816640*u^20 + 1031541996080451213124281554373111041670212501857870103736316232828544*u^18 + 
        1004653602136882143658725390180324254993619889046707719113640956609664*u^16 - 94956615797725279130512836817582682745211321334410609175257859318019840*u^14 + 
        1029846580314263564925120964659599085459463834405114805890708474710355200*u^12 - 5108208857576251881253497866491668383894635359967873427453165275965984000*u^10 + 
        1165234952003913576667798312674107216904033207921689541057587466069600000*u^8 + 129488657231485631520584198291775196076118148634159290335411850774848000000*u^6 - 
        701887827648963911277004931921662462721143013636732954260503176113920000000*u^4 + 1571981418105306169307617174814960909564609634639945156818516838018000000000*u^2 - 
        969906377410702468994285749649313836630627657252872890990319741350000000000,
    u^86 - 13982*u^84 + 91055155*u^82 - 367488003468*u^80 + 1031876118437739*u^78 - 2145700563231404910*u^76 + 3434574051591647102925*u^74 - 4343530302663211742175480*u^72 + 
        4420737961004375100020033970*u^70 - 3670428426846277274699742041460*u^68 + 2511510348926645815781185488669882*u^66 - 1427317615847310216069274140561024264*u^64 + 
        677720761628936488418280085407214962630*u^62 - 270073046635805745285043884605423371671276*u^60 + 90628286079826876086775105528345951763680458*u^58 - 
        25670056646988250274887468344322880048887981440*u^56 + 6146546910661539190508833197010935616776150481125*u^54 - 1245110136054219287360994496312267933303027331017590*u^52 + 
        213393943436915494393103776572856129099541235083992935*u^50 - 30923502867270319854503448478666051302953556918802884780*u^48 + 
        3784224274327350375898219045229145446923452092002571620383*u^46 - 390309535174326538603842109075009445399681413074379901217126*u^44 + 
        33841730689055664349529047899953607613186034004410006604036825*u^42 - 2458454322524176068170239441609012029608509337798913979208333544*u^40 + 
        149023560621788360890885040802716840607305016020630278779853587192*u^38 - 7500143223947061078618233581756687413813159395065451503235249666040*u^36 + 
        311531011845204647668313275129280539365675621361397132552552193452700*u^34 - 10602048656446300034875188076733405242020530279284552521291105393347680*u^32 + 
        292958080212217467549421264717473735738486803443779712762339122670994720*u^30 - 6495248719775032385844896651280682662341650586934296872229076789034509760*u^28 + 
        113578362246266398007555682254422261894498509166650079471655789307938301984*u^26 - 1520873550918225319117099075221882782224886393174668948856676572303700688128*u^24 + 
        14599544909901688146140963137740279104488836158100454146243513814527560912640*u^22 - 79538849829939426129764916362076516577637598065665948250110012335935116307712*u^20 - 
        189814374148668693571614194277507633928438251338856412270815381262006870971264*u^18 + 9042330537926547715916401911482772083112790136958275361584418878780418258032640*u^16 - 
        93159264842422003404550548875038875397752056775316249312707005826585879963552000*u^14 + 435875762284638842004943715094367553574692818094932916195438303435024979829056000*u^12 + 
        264678473399969651768711058566054143645763440065467963185231064541698929063200000*u^10 - 15551259266621547358330201220248117379514469535854666332376594976828732799724800000*u^8 + 
        91176678874325443041621510839456430426863736008217911947473289698055337392800000000*u^6 - 254594792389623438338822446974206617117687505058451021927369242707317124181600000000*u^4 + 
        288543633316807464866206282388698010586434700825908063639134198937120457054000000000*u^2 - 110190375775734617200959877206971752825036611804551201485177232776623500400000000000,
    u^90 - 15879*u^88 + 117667755*u^86 - 541460467861*u^84 + 1737081484806417*u^82 - 4135781626387542351*u^80 + 7596538759170306910737*u^78 - 11049327978328236055269519*u^76 + 
        12965195396629456789467963240*u^74 - 12442000366191763014497990417280*u^72 + 9866586556704105088559936225220402*u^70 - 6517338252137211597419975277796446798*u^68 + 
        3608186865299176058106328140057124092570*u^66 - 1682349296524082944072862790317240454758982*u^64 + 663085463517844097896602475175949303881564514*u^62 - 
        221552005841624748443096402349331822001398024542*u^60 + 62882418685892723621031094742286530624611101447009*u^58 - 15182172819082849033439644557503608253488156057978743*u^56 + 
        3120550498606868106016900253036645204979541180052335455*u^54 - 546158597301560035738930179912888812820256985456195303265*u^52 + 
        81369395473822807087178409819814780749533677322860461043293*u^50 - 10310817934903899594810409992123361682588292933853975496916867*u^48 + 
        1109730679052386435031793332001738263831190184797656454302204445*u^46 - 101250195324582403092271786316539255260506632071916889143611388803*u^44 + 
        7811449958667810988872737833866331032428370434503682697999680413446*u^42 - 507979263593975506472582416858357786192160630182647728612891016748338*u^40 + 
        27735772847830564578516756561333537865659418340559168817339461037902996*u^38 - 1265438634111254982788263165485222126064370468468694772261893638257277932*u^36 + 
        47963795164229654363096700303587442895853141514977493293331873380323215720*u^34 - 1499388189378648000786943303860535591254763045298246132189611190613834447480*u^32 + 
        38301245632098808486399800017503959455041637710474457207408816278675893462304*u^30 - 789409384954262010378932985786621406625483712834057699254220382601300129055456*u^28 + 
        12875204800879374777457371023298906306312271435818365871485825649682882463436480*u^26 - 160353636305357226998283132100793114549117548288111301817631545638939934685783104*u^24 + 
        1397613713537607982464337311280525525456284010137614027775742971777507925636261248*u^22 - 5836751647091026735654707847653120662608723239580269603871920558958761257194134144*u^20 - 
        45975110661889534584103151270371927048806607055220338275006102671984019858710676992*u^18 + 1093965783368832203010414543984697882094463385458538488522352359234823468739975314944*u^16 - 
        9578832022318239723609835228537822888164969679724122624580732987557647605435326775040*u^14 + 34016034271336203826935014768450620646449270832739163231026723485723726793722076422400*u^12 +
        139777134319115952099131808617788897874670179018858356865320139501220741220424781504000*u^10 - 
        2288471260752744459922446049344893841904337438281712434647672372311829668774140829760000*u^8 + 
        12457397012237467486654023385812767617847842304603650240982154626603960298773530896000000*u^6 - 
        35062692940392184703264702627966690910099502917986147621256469063438235618740393200000000*u^4 + 
        39596204688338956984997913604541330603785827388038015573995259323866458255274768800000000*u^2 - 14867583105696241215956713113805947997408412415408743136494473976364029037700140000000000,
    u^94 - 18344*u^92 + 157700094*u^90 - 845652600376*u^88 + 3176564489025110*u^86 - 8899822581241575216*u^84 + 19337871438759035504664*u^82 - 33456795374450624663312064*u^80 + 
        46964110966940465456650153911*u^78 - 54235962432148725419778074893080*u^76 + 52074558122594101113821434552572342*u^74 - 41909564856591192033763370875983326328*u^72 + 
        28451312918355893888953275708072400904568*u^70 - 16373562487652909504014318198646585278252512*u^68 + 8018747224386656028345771910542094282613829000*u^66 - 
        3351741450202435169214851299968826934773374202272*u^64 + 1198348054387559280887635016576098217615350820839743*u^62 - 367034160289045388152924960064967934763066215522478808*u^60 + 
        96394215406070982156782050809728410904662577719215848682*u^58 - 21716857022370996505878669867699979822774097682865238412840*u^56 + 
        4196734431053868889048792621522723210310077747419516838887438*u^54 - 695276720944976079821827709591779953202118914094159255436756912*u^52 + 
        98650467777318791763363645881322441649950300287216846006740269432*u^50 - 11970131525044800266339151896540822867855784754894310762963292176448*u^48 + 
        1239690779149410495284619316988921430519097412289418437028202609603145*u^46 - 109315130660455474420973670294561850554468724389932818113258737841474408*u^44 + 
        8182767858415044745226661410710164974728229233199030294090034639204097122*u^42 - 518094937674378855801018091959815445716214235233799156271652612612222826792*u^40 + 
        27627384770054831563799103207639139514187493116781908508154242052506796818628*u^38 - 1234414193971508449661057293792151977293702263041320922633718011169599554127680*u^36 + 
        45928976852416303640742237756029627645273675507781849102165887730089336633195944*u^34 - 1412267537216833865317636021367193404096493008375311219168992577975009857465912416*u^32 + 
        35541211553287334580299223391889447826111061354805383910392385378870507097307114656*u^30 - 722328932905189264782211429600647537277339421294552436939956380175381650828701905664*u^28 + 
        11612170763922515981678345294061849249844345497840912555408975484459470540334241997120*u^26 - 141982634130689354067248580875263119184722226889673431969866332449716755277440624463104*u^24
        + 1194134194832885726045439618007647003463213447364553019728336828014988725729119350804096*u^22 - 
        4190368544853718193197373340293048767619600579111424222650016756941437759413722099982336*u^20 - 
        54102942455743337383461811947454107188626690288358775546459382586495361986762126331108096*u^18 + 
        1082170143351300522428346789843393443247841579407828955985859086734485859745846032729113600*u^16 - 
        8760557083769724233210130823014441930639904968246808812899487412310955722465509607426937600*u^14 + 
        23314206957050562914056163508142881874292189847459295415755257562277243325695398922659584000*u^12 + 
        230757338612592207818839142975179093449281297396518218225859852608708583446831280546658880000*u^10 - 
        2898646796076399623328772564423797330488276533110446356176078722057643410402603347679520000000*u^8 + 
        15763172165472855505433310873140275729651284157084583588216206982694108618091736853583440000000*u^6 - 
        45991958650689403919457340080294233778152266498294829503198290269304155680688655925113600000000*u^4 + 
        51730571811698052464255084308457303294807730021724405868004765980837952677894942442804000000000*u^2 - 
        18848471307193436782010069565608353983482648244239725045184871605450310265485752439600000000000,
    u^98 - 20721*u^96 + 201674772*u^94 - 1227310900196*u^92 + 5245181043382722*u^90 - 16764203578813178706*u^88 + 41671001769471160748572*u^86 - 82723831392375376240998636*u^84 + 
        133662755297627177031901719207*u^82 - 178276782291596623141862002225671*u^80 + 198408034395957673425067001511205968*u^78 - 185799754805910047788396728153871424592*u^76 + 
        147375680229353303025654630715237728854484*u^74 - 99537200839848441954117839167644544416647412*u^72 + 57483352545620195748194469598756564230868745784*u^70 - 
        28479666543391654197714644850530068152640575916632*u^68 + 12136289821758873151509556571873553465745493633156559*u^66 - 4457023714123335031665210211894458727911106907361175167*u^64 + 
        1412607130738193942606538941047881543886118157466234355604*u^62 - 386729463308309444510824503974539352310914883711736591872612*u^60 + 
        91494004581337783430148006884329154916723268203915057145968690*u^58 - 18705775068235462508509159394068008185395447620578369784359149698*u^56 + 
        3303452398492457969471292650861646595417131139379544728832566719116*u^54 - 503495842015773397048095336399645969213436741865248746949056814626588*u^52 + 
        66145082183709754328732690052979074541561699742476225606208739694507641*u^50 - 7476826940886118185519641199603031448941761862387406686282849404042063993*u^48 + 
        725596474433669074700496546925314301232042805913666610059999889612858497416*u^46 - 60290918920649795672465644848545306672481803532935546018327741141487150764008*u^44 + 
        4275318762886927951894660255702612297205020108367885727304360598723325968110296*u^42 - 257725331236504691367603010555725833573332950793225470049926406702075959266076888*u^40 + 
        13146791935135274137995052103355712449908411567836381641630206561264259995955415712*u^38 - 564399735787764796233663688645681490780789172516349252889326473755692020554822758944*u^36 + 
        20258977531962987389719484267620947408017187560549221370757723610746446842745113711728*u^34 - 603151270591633598019622352539256166747206946587859352325314721544613061104772655432304*u^32
        + 14741459644530505343372386758337734621763403858720660967547776013822440681585491203945728*u^30 - 
        291571248271230213240567033607426091436224647684184035153646202990386815353463360808972544*u^28 + 
        4562091455759905530244847011675353910050843754994938741457408813263328606800103715745859328*u^26 - 
        54010428842168186172410930981599338781174281465504502885551020822345944663989235615064504064*u^24 + 
        428722736507555166708901072188705742592594136114377264829729227591166226615574172862488096768*u^22 - 
        1076944798351949281234510694850436487872824405377694220715747447620363901828858310721535176704*u^20 - 
        26726854517915901222112945519486620798081799744034898871020191026940034305829864610108284938496*u^18 + 
        452389719876840387753806254642161434857024366684744062962400469766633841064609178776368235342080*u^16 - 
        3288512662577270198203035869717272921935613136144865952719703443296522180508780676583792031897600*u^14 + 
        4471116902208695361250131047024427614505798924132312123034974298258176009706539103025658188544000*u^12 + 
        142392642538670905363905630783330427072483224712452392673867791827183314663643703273697398972160000*u^10 - 
        1528482635846115610540092146265748585001955936684551295233223662581481579782849460126855764320000000*u^8 + 
        8342895025200547605806388413268535737995050694772321508742599915722228713390853342448647496320000000*u^6 - 
        24958425789938208451094504421930580460661797203043895874046752258588427979494125742546977718400000000*u^4 + 
        27378390101170714518582634615117791393275086099222030575596434155514375332712383962037961512000000000*u^2 - 
        9375772294440242345356274053743637004094081265094311200169699311007274881401120375526837800000000000,
    u^104 - 23675*u^102 + 264225079*u^100 - 1850864669525*u^98 + 9141630119105710*u^96 - 33909807568800196250*u^94 + 98260984461429186431170*u^92 - 228452214069016789415214950*u^90 + 
        434400116384655744257307426235*u^88 - 685279173335716239430969688660025*u^86 + 906737376764662562906607341794640901*u^84 - 1014958011675536188336845857032232699775*u^82 + 
        967638768784216745070244980977722301789364*u^80 - 790010632405097301576324777615756859590572700*u^78 + 554750725495791915852144846730812649214926175220*u^76 - 
        336219500443707711888977016624889583891254698469500*u^74 + 176364664236447126911233698269741101344955249531626615*u^72 - 80242410608579521069702711936864910781729124903223796525*u^70 + 
        31718461284204207285416162356441732830595822633693182870945*u^68 - 10905524971133189605129142609392613433457023977712341824530675*u^66 + 
        3263895650749858187800493204552763127211335684828736997336003966*u^64 - 850634492141849883368434251197722561140127809401557666326142466250*u^62 + 
        193050919751787093003153136843039524161561962412554887729291908357634*u^60 - 38139792998828070151001077458857663629860466967954716275454586846571750*u^58 + 
        6554989994953836881251429415886143351091230916020586246948045406102835805*u^56 - 979080092734646933873712551201283083110692318209932825395205791620973615375*u^54 + 
        126921855695348954907797977633151056025204569766296243792929224916339577099635*u^52 - 14255959759071220596178412655763669262903883567817139234493825414332599971565225*u^50 + 
        1384559485639878925763922383939978798581637323859806467254889993139517808011113280*u^48 - 115991999595365741393728502671316759591247233221876912028853745425623997690673199200*u^46 + 
        8358137727364406394419863773066700820159998459969846610501771617550509165219539565736*u^44 - 516316164394836019902982745230414727264082072099622451048543302040743188471416082976600*u^42 
        + 27237689703968639405773259873200646562290768486026612029552857806465962020757172815615824*u^40 - 
        1221554446992141964477673789701034496393568572578972826640304602000041303347237481148922800*u^38 + 
        46325804270909405531902092211755085913462957479634995526297547019856502134079921839681410640*u^36 - 
        1476014470871321606309317129846801021948204507062930829337122603743901665927799976608350982000*u^34 + 
        39190059442654518064571737731995062330993579655420486736524881695651348906847527751301734030080*u^32 - 
        857664315994165775025806032181468939921260241350979426928800627670207000035662812182254262860800*u^30 + 
        15219598497613424985720332506464961235472002768831910192953785041505836095868716595897359265527040*u^28 - 
        212812741976555578801169420971292097340914979350110955152629672168533310714915795518024558258297600*u^26 + 
        2201256247960834762225927917621482463865540198059535571214882129648912584136211856198869844816176896*u^24 - 
        13660228898984740051454153597159567266934902890780238710306911561294894798969481969403887048562771200*u^22 - 
        19414016560653804123585201401226360767554795572833496620239178877841668871770508344751991063490859776*u^20 + 
        1618964949356442426292566856450071681612722178580721881618066894224370654083669316973277969660778502400*u^18 - 
        19385534813283961799797229186600758130075660328571628425004828747043778990569552041761596641138055168000*u^16 + 
        99891762580027461523777095916574945228285963999953573552981081808068808313001100369845319679514306560000*u^14 + 
        287513541382277462963766011590656594016801086616977370074746078228684033905720906971221607311350944000000*u^12 - 
        9247562611954003532338082971037809289097029104561090772911847586296142960748925782657512653160965472000000*u^10 + 
        80686344792487503883982315225980524390107865079221428337039681069058074829767077975288356354217611200000000*u^8 - 
        413052382801809809217349029113983082619178941005871157735208449340162981330836009299347045311277928000000000*u^6 + 
        1176792525641118218372025154943724063477362700665980262957624459858693477726576526105098089593696120000000000*u^4 - 
        1197473001472936020337627824930618376317706651972944518249531850969022618383861056335984703209988520000000000*u^2 + 
        361490618589262748159988741873262989034113920090501320896646830976182732430684362973573853858928000000000000,
    u^108 - 26356*u^106 + 327905804*u^104 - 2564177613124*u^102 + 14158768506761735*u^100 - 58803570045840180760*u^98 + 191074953003462090822170*u^96 - 498944150513610380501605720*u^94 + 
        1067321115826016713883856648185*u^92 - 1897427900035913670491927878940060*u^90 + 2834330473133230119466022176310245176*u^88 - 3588460444249254467039173309007827069356*u^86 + 
        3877336352422158152633040465617874490391439*u^84 - 3595344258339269627029190692770234710098638384*u^82 + 2874010806131172012777704075497369133444390246670*u^80 - 
        1987796152914961030946052131254574200688457511510320*u^78 + 1193126804778760752813508451336959274518804877773088115*u^76 - 622985931803054160236439482291553217026512880040946759340*u^74 
        + 283516607437966191548323432025340073931163923667557939660220*u^72 - 112624450960515655625351763675542149717832973489859256692712220*u^70 + 
        39094910477207280835713430376323915569816385104148582426755228141*u^68 - 11867795350118997494356790218225302245601489392703354883293107667096*u^66 + 
        3151895444220691896169894180518366687911379708742959498827091589070934*u^64 - 732459462877458584277188138500370711615909674120949677250436922654985304*u^62 + 
        148914449199954491053647870756449974585673179992313066490261251868553978555*u^60 - 26475152876840111672426984129553327951152655108897053886027045720292609544580*u^58 + 
        4113113926894250260299172930751569368115238741032603585825927064351770975691760*u^56 - 557812881601218164288939909563180978055800318938147952486271324889567400149748660*u^54 + 
        65949938528578038185405682593488755217303974695929290249874473207570371825022197005*u^52 - 6786263023560535495621375087166960754943862422609199305854109274074549177524042814880*u^50 + 
        606553133682294547646809451839849733268728205576254515518143960142826531060958909545186*u^48 - 
        46978027884055004994990712893622613293025182794998142414718610836967432266938342392486816*u^46 + 
        3144048923753825384029127488117868365777789583704066632143236270311153066862385034386363224*u^44 - 
        181226436008951688384363041294857749041587342100460652272174167227073118421859483157096983744*u^42 + 
        8962139980263930532313634816645053008276432154091165185543606820321595324600428232190507855440*u^40 - 
        378508745133779401073613923238720556404570507804192773991582023558365790234159482074188382203840*u^38 + 
        13578104979985472843660522955830892876625248067745088413234154062626931652602243084308278170916080*u^36 - 
        410947395465283488302392390004679643876860107463349501784196542047641961363781623076772694324961280*u^34 + 
        10403528963942807554450531789943318500668331209794661431110736229402523326357485321587050564575775840*u^32 - 
        217710032823314637297631938220646192740074679697354730826684746742863308908250416880457299000303907840*u^30 + 
        3697904030530324598771129870606246695916706188460601920671671231993824135692081105200557804780755306496*u^28 - 
        49316602010888421992470764274739628919689541551504447097933311565864245478235289356850828801394420325376*u^26 + 
        477890036303462518244424364479925471947323130121415556265388961327557639535704550324367074678760948084224*u^24 - 
        2508990820889708623162059834621522917452563993280976776418381799887900487251699589027333081252914813266944*u^22 - 
        12192555418681694400119654294311753382644372885211754036108599522178130405815524232723449895790046270342400*u^20 + 
        423975746670795560967332239157980508287742354752553183346361065742495494179349378397354044829897151818752000*u^18 - 
        4383841517224886112479596248682232263678475730890530113878865597678540709822885648224250107464690613445440000*u^16 + 
        16451029875685331618758227607217022437115417100710432396942778883368769142097745469888983761831648280755200000*u^14 + 
        155320064739527151027883708047972498294979713452758630585431122534697526777097370379714439996059268678880000000*u^12 - 
        2928123026591035292785003318233082522119174628663526381930773650823204088649172036050685274393968325356800000000*u^10 + 
        24176855605082106345268627592354034795455156490728148057430760402520823173008089710102321612127842830664000000000*u^8 - 
        123687912990832143043223385931169513011197101406197576875167507539072524815549188333280409380121191334560000000000*u^6 + 
        350001751178404309117652299360319193223160738673303275721944396526834606474764570007672412217920776903720000000000*u^4 - 
        326603292279910255112795706014722261098768576436389080798627476955765307140748308374781288472807959232000000000000*u^2 + 
        78461093082136168427872466777847517833384000980008634505069577999307616380368663197644756688263339850000000000000,
    u^116 - 30023*u^114 + 427110847*u^112 - 3834431464809*u^110 + 24411208291518183*u^108 - 117418189790057211273*u^106 + 443986212394598533471479*u^104 - 1355901403620476529076842105*u^102 + 
        3410114104370241665006100200355*u^100 - 7166953971379814348189869227976045*u^98 + 12729854667040825678550942992495742651*u^96 - 19279789302826355899787049659266841587093*u^94 + 
        25076956738539321374865042491401821139349667*u^92 - 28174931270987278300535288307287464485574827789*u^90 + 27474689142100586526658379252963947674652900492323*u^88 - 
        23344592570860356864142203469617201505371951090896973*u^86 + 17339108443751702496903509683664979169112378669775660489*u^84 - 
        11287781565389154961764410456729303730237189554874014754135*u^82 + 6454677138017013810704542867540622353108179751567208140616685*u^80 - 
        3247760174344371219750523519388576217130694737550107997333355315*u^78 + 1439907925767930882293408946340873769542934386405890099352542047541*u^76 - 
        563092587662732001740494202098031583873015820588163769865635569984283*u^74 + 194374864562581731549819689183786887150109911422929353126845654245476917*u^72 - 
        59253506753376749752462450177133027244944696259023325177933598096304021979*u^70 + 15954559547503001093226616247118710763427753211902890392861620488577758980433*u^68 - 
        3794243756389818150481418885018737101574225810134270422472317368370835143914143*u^66 + 796711347836388339209417945991837248264646905351665000371396395950097627514530409*u^64 - 
        147629213586562120365466542381137323663173441479425146877921071358319199695415897415*u^62 + 24120917137691920376963060951298225917648721831962317575116371018801566621986337744065*u^60 - 
        3471469556942195401497351435650437986091379914257624203409978208800034783028262878038735*u^58 + 
        439510328876592733752583436421223742362697255075154320933630050231327394992996359104216961*u^56 - 
        48874808456908924731444003802386638773548181374588379253777283344337001258833201618237930063*u^54 + 
        4765024716690522014190722867592755382191015189503233868027513643411101125345111073536843834402*u^52 - 
        406428992569113924061424482638538891998218465379489759605577171354721858130741233383623772077814*u^50 + 
        30253763140575555508878410312012320521374892198537869840241417637682462897628038830827761035613808*u^48 - 
        1959885539567389743436211711510942568313676919410687878216725549499188223415477220455543979276656328*u^46 + 
        110140038090932555603475118019796919368348792403361300790490041877066935415969089049819281797525727424*u^44 - 
        5349653176576154093970235626939813581704500380102188167297925004742578414548868004839919667022678438720*u^42 + 
        223628213643453673788543222292085854317395777305125304005705806768050721203297094559879274622399215953520*u^40 - 
        8005411777655613038638091511926474101354414927003399977028074064530372423458167518679798538252916961379280*u^38 + 
        243943725620355759068881497798933348351018249397763173459815392465205011461570424675841042964425094315824096*u^36 - 
        6280027136776340347725025943075313408545144013860599207341812173879675666487271102275259878451604735488912288*u^34 + 
        135195610929668407924943177865622559474442471985342962985606784346796323935047615496931741696250528971033393792*u^32 - 
        2396769221914387475543645379243872889728959657708829778985473991104043241949209330778160152294884360970145641984*u^30 + 
        34066086200078032403618925843205518080475245977696424368543761246785854946838951918420594857085791519265091792128*u^28 - 
        366464580354966578741959257232063190491527497786462188610875320158430241004029759458545216500732394468993595249408*u^26 + 
        2498360210457257737976421254807042607532586377831853860403819604438361972550872530894537737353516607596902762925824*u^24 - 
        50517980785310203363875096903694363632961275421099673748028344862169288285668900741429202776726061319558747552000*u^22 - 
        255919458128301111642779507462209070971912532104865707562661860877803017830311548450374349797145962200556989538624000*u^20 + 
        3447834299984158421283620132130225597026345437160917011650590757846913541617416463209235921925337480689824407816640000*u^18 - 
        19601135446698199555442448767924996726593247695583582217565368511922444481713073824165326328661140664225008864793600000*u^16 - 
        69813830390295266835913815963531520487174054671103314441909119594440808299813408979265306177712960076201290081952000000*u^14 + 
        2555502619529426406432745800025733375163586938675197498999277542042355395001799260365071199382467551114347887011200000000*u^12 - 
        27553322938772306408508527232881604072818739101001687599197128113030057623795021445740750380855249247903766152464000000000*u^10 + 
        185095173835046200691363176902822242004278743260707608164090524878542734646769535120716207639300996540231688879400000000000*u^8 - 
        798395262448226865355744429445046154202438036482045931761322634092386647489470927999353145160074059035931040947320000000000*u^6 + 
        1866209138010069666135733119044839774287455104676816494763362185589148379963808856381149511305751199726144856338000000000000*u^4 - 
        1417598762220223244995681312833127988719285218458488730285102542018240946625418856309800829266679081590701278550000000000000*u^2 + 
        184659361729973474180934969173584985269598143697625292367373033104526041339321003036951580881107365694239195000000000000000,
    u^120 - 33048*u^118 + 517930476*u^116 - 5126443558120*u^114 + 36010391326838820*u^112 - 191262369917849428296*u^110 + 799178163478169143821288*u^108 - 2698969901058960330526565256*u^106 + 
        7511758353543852547434053452260*u^104 - 17482692165048368701768182773720680*u^102 + 34410286927285322546788703908776429336*u^100 - 57788518412578034720110812070130056520808*u^98 + 
        83400118879809427958662963567112286345015856*u^96 - 104035731148717551469513812296613838250954523240*u^94 + 112708168119911989743552463351411918644661789813800*u^92 - 
        106460870260891252242589714306524692413825315064911656*u^90 + 87962246771344554996421759489905439120366907802037954398*u^88 - 
        63743967618154360988180682295457686043200942685063496681336*u^86 + 40604623791307863916174675604656678252622022428846216074976880*u^84 - 
        22776320435473037723876922874540724322958965767848831861549873560*u^82 + 11266374206276488246639621444421274337754349439625628310839950355336*u^80 - 
        4919917545860933625758829644991035812680012687768741486366353748732888*u^78 + 1898268342104842068045720842118636662018662111619004451652123605815721176*u^76 - 
        647469036184657699092500418835812726675325560000756849946322650434814907160*u^74 + 195284268719762547390034716989584290193380528673327024735869702974836921311780*u^72 - 
        52086196246657877896314773123967417198415116433587138672489283148199745542212856*u^70 + 12282987230824751565593990162069064309407996489620104722399032271990115110032205928*u^68 - 
        2559945849633376293065870740580193057598788613961177105894991709473609142742513384056*u^66 + 471219959260498383044778524383501945092288375037770409784818396753201940705754806168400*u^64 
        - 76542741737976807089551637112894387141761880516412876168431704644312935724535263440606840*u^62 + 
        10959527596399998014507353970033132110732776246978582715953348174206608829337719737053733816*u^60 - 
        1381346779179043934458247632801010391847239465404623928346642951435584156577659879797466599608*u^58 + 
        153018236284300775690406202588478683868350710037131900645370008801447178802119441141687339713801*u^56 - 
        14869778572522153314215529997996731322377521988146889645990315409246002460252073294591197826718480*u^54 + 
        1264894863238877671582253319569112890737001780602246938889282573469917450523133968443751678476252260*u^52 - 
        93956430088285183701470043290181768650055993588662047136396260549783353640582263871346132324536511136*u^50 + 
        6077229471799540695362993096002135916941210605360326746349220871910291391577328343817937426390497718548*u^48 - 
        341199432070794743508121399070042838566905687938081323535450102024771966229483351600868211921356755961856*u^46 + 
        16567392301708134469942484379429084752541832861751929192856549183327197187356430051011651541132744541383520*u^44 - 
        692823777446210510576790207138006489035496845333884707304295112813553319035380886889494258478121766998017920*u^42 + 
        24830371715081451789375179319618829859327201229977027462614856387270247875889729237219660047378668003600037136*u^40 - 
        758176173388860634959662266332913866712204841440820384677742595684373639819973387114456731152486905029040763648*u^38 + 
        19577095206899598179953531526831888523905925222262704464672841354274717155663867682119153121312931121560305146816*u^36 - 
        423180879522622299736458209905884850797887208741105653486372962833984660184634191356836079150916637121919215168000*u^34 + 
        7541482158969373038709604863571194220320808286410309051209413433319716991854719087787935454512682149584012399595840*u^32 - 
        107856395052896220169569331308393933460519208835977306116191292848713177041591167589874427095555676687072369193261056*u^30 + 
        1167741736380513354349843912195968804349221925781572968471477314093791494224094217436094693137033064811706278574681088*u^28 - 
        7984785227675039388539804476261646106135892618476261948978665260870308330247957611140726379666785124685359541509482496*u^26 - 
        1001033765191040694428141055090269332288664252902749858355722256644389231313788623210924232081137536528140176104418560*u^24 + 
        851602997818558853390795276919516938532495176592982124038917645576000240294129705724645989857442138824036424281209344000*u^22 - 
        11341906122543884106872787976338371187710403818980300118231115297707388538855632738452172600389690431824394679882163840000*u^20 + 
        59608595977597595017057149044565818281110511741466211224275816596582671494207693392528115871153748309969758860215628800000*u^18 + 
        372493484433837394996520755813336197734151391044636744711738447417498497049764014862144858691244078470562754219259888000000*u^16 - 
        10843118237444123021827174679260861381589742592421083216565223461038227677250227367136366861420996623416107926743915520000000*u^14 + 
        119562406741040118783570002338401550131115712692847995083874161993308625846241111278630918047342642597037069016311408000000000*u^12 - 
        851959443631487463416914834468223072416056350358366608110021194432576146776894631012505693129639613397767800036471360000000000*u^10 + 
        3990891698524718134896930747522019900717685071465787864707108718054467699014530495483288716434416271016351390123076280000000000*u^8 - 
        10685602129067369587656357163250696485363226112949190767341594551014039089726139571015028632068078075160036906643715200000000000*u^6 + 
        11938494607860541016277200144813354199367908189105704809953943438225260791291789727463242556929708412001635552414980000000000000*u^4 - 
        4114388919838437222126828087631419528795809633023949879724583684855496397980360959273835993784202885319198478588000000000000000*u^2 - 
        386576679815186551146282290066866491488398314406000062675472896602998854784919172967271421375194716592386823362500000000000000,
    u^124 - 37025*u^122 + 651726972*u^120 - 7264396216444*u^118 + 57622884975971468*u^116 - 346596577397352806268*u^114 + 1644967843119137675811984*u^112 - 6329483808744981231592890672*u^110 + 
        20134892270636980234196764053420*u^108 - 53737247445319195060291548990062956*u^106 + 121695561458595442279415504567080918496*u^104 - 235962005398236326425537518678970162636320*u^102 + 
        394554994821337926337345651500993494589074392*u^100 - 572292953058261345669647505249054507338236051544*u^98 + 723546213644407487661003309090176630446157301925008*u^96 - 
        800531902445123139489644012748264024925799451312429648*u^94 + 777653253990515301186344497831726645293101801072077860294*u^92 - 
        665077277176579925794745375169759763005102549574509058330182*u^90 + 501894291407990302456931541598239075037354962340850417991617400*u^88 - 
        334813154859845997239295874843985612972759547460747749655493664696*u^86 + 197734541391166725319537645405214355328053504006853156884546072099936*u^84 - 
        103503094869563261298439742721825749555109953722029298721910556857944640*u^82 + 48060814462018714573288624439176031303929064554087117416935400283930762992*u^80 - 
        19808802454678902329989162632187590390587432477680872046539554198392026718704*u^78 + 7249555994400193839267271637649267778383312175604596284747839120700891018076668*u^76 - 
        2356179335262843747999277214563169687585785421660559018100237727630282903653557948*u^74 + 680005194027484761017442537933184734235189609754449097314856875292109444772027126464*u^72 - 
        174218813853024390091806758435161246540109258473150587212386088774089290047401050988672*u^70 + 
        39604039710444278932089699164336133528945386566569070149485939224504071775299821397670280*u^68 - 
        7982512934514160997188170325311628729275015481495375658243285800105385514480078995304055176*u^66 + 
        1425281332459127682519457335760546058132168656191319499804562210420272576400344189690841553456*u^64 - 
        225183728894235853707626040224515911318884411138111798491751350656698965284196569102963187906160*u^62 + 
        31439117751610572409986714360924275903178524253825896035315544639550858856270686402980299718408577*u^60 - 
        3872800732151879402001152299258980429708679247174232742414254538618265535443702052385317854683507809*u^58 + 
        420168786208046650588495774417026029482818426920491696920568480333850922873488398184215859456339348268*u^56 - 
        40066344308121942392257993822421893222796520150611826029590859897083403530012043099281465261060646532588*u^54 + 
        3350339119297258639564088536588291113116799087970921545601486485560038018893409951955798534328793912662004*u^52 - 
        245029146439918745655304791755443030844949672047374516231892540646763130145823986456080060321772626793163172*u^50 + 
        15627495740168777638258642956608211749524030034993406333344901593958150370974842645816068433734159141664218560*u^48 - 
        866286708188643833443298859596733773555444774652983361710894503413951068561232493989260953851329188439810568736*u^46 + 
        41581283797990431826951331665771452198993763048943431152961592136493452876221997555459613215937464325301631222416*u^44 - 
        1720763769214395356901119246250723455011552869319996627816960567287650162334250339358006447877174663543980270526480*u^42 + 
        61085722073845967810761229822822585858135597403399607424682290514808846680444819213824866383927493261771078813680192*u^40 - 
        1848899348745179745043955535108227059701873605844646483911996901215887362426603122115714588731707206258825867461858624*u^38 + 
        47347714321362167780363839292603193264133600424738615153929389609613296532660271928098771068541902566480831977743841088*u^36 - 
        1015126615896701165600753873069360768215695638484982835465843020365128244575599362430499563035297367728355600227260586048*u^34 + 
        17928967737749510836794748247703931432217677993385808079722261405899516575829205695094891178298396023704237710015116245504*u^32 - 
        253407399223375767616762529709114778981629592001639795931642182026031497364239018467640721247472104759713487569126172183552*u^30 + 
        2687212215820325445470239136814305128189632696587046003699350752699894448120785147841114270914486460498879757117097290627840*u^28 - 
        17296734661681972028915414561900289849184167558091879304508193346171290207753496451542631661719139817212664545284853958535936*u^26 - 
        25255312832282445150026780600270464579617320016405155026195721527801198433554038884945307326981705526736366097497278357703680*u^24 + 
        2217651669371349714954373476969486880945017222635822008238205746379842668660334938303499617090627489884110524987686419084160000*u^22 - 
        26903152879324675354908308873207339549215404091310789960873147045958351642652476880853442223519025491283308461737781016156800000*u^20 + 
        107467118934785687948472213795827812008121508012410949255970436677897908731541308320149513322416173352374830492378499461609600000*u^18 + 
        1565682542979185054273410771464164117371091380031731891603145274654306799183543118545190964924765521747069488085150009445888000000*u^16 - 
        34571337664024198155604539563697551725631250880151153233193189295446908397418580232233598645959395014301566677909236891384960000000*u^14 + 
        371190032643199390079898006602287847743788808577632249743519067776616908772364451976850478918877466354393093617200193249272000000000*u^12 - 
        2667174298976533369097447192081385227720072294445036592297125279931302055564502612203762979258926682874652579245391350500280000000000*u^10 + 
        12570889476894279829796143465058835130106485370716066213440133064545937472599055285176981453710827446577261093469983029904480000000000*u^8 - 
        32783145929642978345996827496970846639391776629371150598525592972354180937027933643003641338269044833931158094164628131141600000000000*u^6 + 
        31098776123251975177646959087382040169525318622815332186512098793800835621302544474240583237813304902304539378744373560540000000000000*u^4 - 
        2382873270348244059223968664649615167488097131387738692627334340434423218904391946313653582207726641560403980041251591500000000000000*u^2 - 
        6174737640557250375478194124521408450603658763855546894082462932350110415365690599117006196037243206648588167180457900000000000000000,
    u^132 - 40964*u^130 + 799217404*u^128 - 9892793341556*u^126 + 87319124207871025*u^124 - 585677113680667101680*u^122 + 3106627632849445940877070*u^120 - 13391638198683310361447279120*u^118 + 
        47846076549227051206065540345280*u^116 - 143803414184678622114747564586462960*u^114 + 367792720299449822244836949258154217960*u^112 - 807833162721732295572726777916962445848880*u^110 + 
        1535112774057528238080023196231319230297912980*u^108 - 2539210217467499370570855016612999035570894566560*u^106 + 3674417479388916849407867761376651408084456352394760*u^104 - 
        4671382687394283070163686960757395272479140255039720480*u^102 + 5236205787016591533296092849439300519681296787038192382270*u^100 - 
        5190530236971650190204674777289885188018392136205730241845720*u^98 + 4561847257755012813213681471043420290133961654454290209632274680*u^96 - 
        3562414464316735950275343275139944030892379211402992693289094906360*u^94 + 2476378707082840567012001978256550898019526971985464982224757906417950*u^92 - 
        1534703161366052058475507058246689590816440562963657391020557407609919040*u^90 + 849020180637485646713048727945342851858689454758358354790856685484698540340*u^88 - 
        419707283943902047005932842321713407285191335311625779192641536070661487398400*u^86 + 185551393220107184871635732516761126850576433769341753620258962942921414747477260*u^84 - 
        73407116181417855662099868863095746920420937399116095728586130259202835523862962480*u^82 + 25998799385721648272619501372288884565538358390696245058433320451970835656554842129520*u^80 - 
        8245490046595875677450802050533041260718998312835046803463482847696501094936728423483120*u^78 + 
        2341851163746016657683667896325430380369079404950953400308494223214838662526715361367421780*u^76 - 
        595579699656409801383749948667601909585391033093228017292157435118701957287989175748120648160*u^74 + 
        135595058671069175841956143800814222682972245169319866744544492905537930640717081526212824755880*u^72 - 
        27623859631273035359898794188107523828309444137750269767144633911187553075569372504611522895684960*u^70 + 
        5032702998009913607441273186842428962052845265238464472043640111868621969924383196654491011092710185*u^68 - 
        819331886687238104085560339807164213756942010604026375266197377487787620153821039178912899888651597380*u^66 + 
        119082522125277954251034867908500909969654636024872809308183650655530923831543449631669897779195354175660*u^64 - 
        15433816413857289226148676483065336891804280279153944089236199130480661828253899259140658119472280941955380*u^62 + 
        1781387947206247392638150658114471670085947153503553704381665721940700147968650234922924903331486892678042745*u^60 - 
        182825182885084053989117784051164167917397934791228416628085791542855810382190417660018961706101784931423255120*u^58 + 
        16654865129039250526603097114699048392609048931932021741690932484278942484234268712413872176179371561397390170030*u^56 - 
        1344012257539905376203263422815344229109146679501691474672428068230989070722279421631814981775013803722535368507760*u^54 + 
        95859439556404619153799198376318354863714869130416257953517667636213021729795996452410239672193940353566915242609420*u^52 - 
        6027226665650867524122663512773879964474751932624277731948317835933989392595109328559527464221378750520994901385885120*u^50 + 
        333106047226887636403656624633793836642615429993526639300903868776742265225962593356446344848440704494570513427702550920*u^48 - 
        16128161590405714047813338510767430383199867972609001644446157688251869364561103318920371591933712761598651443378581523520*u^46 + 
        681498248394555784830206979537583686800895390764421038642383078090718401663068824451108024002254022122587201775333860673360*u^44 - 
        25020016835906300607873718920415125037153640827334528855752158217020829778453385446871613260731435149439124559100440208436480*u^42 + 
        793860261173006080742200982893503855476808465511518668355501554744258760812146862730085150420369589617814778627014886995111520*u^40 - 
        21625684033915861541705370510351501314264474212104450817533505331847421500523009634067228221812755409665955599323858079731761920*u^38 + 
        501413635471951223648125979762109971751657906325842111120205127262187652907012367314980275687381343166915866244207160413534444480*u^36 - 
        9772686465732257918980126829633082531894610504114110234192411669081228884780640676658566612875289264585301728394540717882815349760*u^34 + 
        156915870900472499137806005350592727362930193479050755593088908547018325519659532457417216090037014228714230683062538137824764545664*u^32 - 
        1997371615315698280524614615922210846292624792126901897515306980457047197081822690403062508968600042258191634458828064156456106433536*u^30 + 
        18347123851555053181330201935248120253742816589959434693381906024819710641805864999681728938268948576287352254487018194886603701271296*u^28 - 
        81355726421158755436486943600802741372489137901953619843641442732039530605571580748963848543081173961581435467030668298457987354947584*u^26 - 
        759724548420892806285554090948534929508250929975265934762628938408118191915523955744657415015824213120201570781260881466375903944701440*u^24 + 
        19198398222778068006034862612198769767907668526570069978680685995387669211316933488697775658651650535312372512550510635462647316196864000*u^22 - 
        165409533953796499771660048555042509002622174716776713248436557195128032136799387375635910574699005093346776861486473330142466182547840000*u^20 - 
        127727771648249485008678299296942311015762529809759216373006060695307066303903074654288483911050798481491710117366591653685782727936000000*u^18 + 
        23376524160346645961859758746031423625934491631220121115461469423676459945549074005584803261859579943486834560804626757949613003512672000000*u^16 - 
        364911019635649696335611223259040175954905764819031806218332805190374344487257447511361025564192416600955135958198554455609727518606080000000*u^14 + 
        3539706578469094322336734647208481293305919761830901426649209714236395246119268730041778629971515930010755109109072923829259734811736000000000*u^12 - 
        23940722477340318039721823454553336412443823381281979570623846197801303957857248013548522949580374120517044895777358157097383959643520000000000*u^10 + 
        106020780307789734634444336231307742967065864770361389462594228126810791311975839816280625995194023436327857923449805804698080491898320000000000*u^8 - 
        251355287973380132173678364484087211968427854375096728503049149853204150329031473816477527663331037957544777636846815822849438752732800000000000*u^6 + 
        170654242805871160094531873497499721315176397943437661810272286616924239752319599025530213680085048648122642635617651079297028921220000000000000*u^4 + 
        96494353232687827989929864258379195999010341266000243481304342999080162079916142147027764620241090184777029509812796912680174768000000000000000*u^2 - 
        101071143680697489585945989844381376713458731449100360323944268335437546363973687869898165609721043879765192309933357903163858325000000000000000
]


==> NumeratorsNormedV <==
// Moments |V|(2k,2h)
// \tilde{X}_{2h}(u) for h in [1..30]

[
    1,
    1,
    u^2 - 9,
    u^2 - 33,
    u^4 - 90*u^2 + 1497,
    u^6 - 171*u^4 + 6867*u^2 - 27177,
    u^8 - 316*u^6 + 30702*u^4 - 982572*u^2 + 6973305,
    u^8 - 484*u^6 + 76902*u^4 - 4461348*u^2 + 67692705,
    u^12 - 766*u^10 + 215847*u^8 - 27766980*u^6 + 1653656895*u^4 - 41530140126*u^2 + 337968054585,
    u^14 - 1055*u^12 + 421093*u^10 - 79486155*u^8 + 7242179715*u^6 - 290444510205*u^4 + 4099101803991*u^2 - 8381907513945,
    u^16 - 1496*u^14 + 892108*u^12 - 272180808*u^10 + 45430344630*u^8 - 4121412379560*u^6 + 189676636728876*u^4 - 3674923533427896*u^2 + 14539253947899345,
    u^18 - 1961*u^16 + 1566628*u^14 - 658984788*u^12 + 157743552510*u^10 - 21750520014270*u^8 + 1678578114026196*u^6 - 67707100461703716*u^4 + 1235110338400818825*u^2 - 6787336148294472225,
    u^20 - 2610*u^18 + 2860437*u^16 - 1718473240*u^14 + 620475009522*u^12 - 139083336332460*u^10 + 19348398203611266*u^8 - 1624490941247619480*u^6 + 77190294570345945549*u^4 - 
        1813095317449668401010*u^2 + 15009483262024846096425,
    u^22 - 3243*u^20 + 4462647*u^18 - 3407674501*u^16 + 1586340567882*u^14 - 466277764083726*u^12 + 86845227411024846*u^10 - 10042821279688179978*u^8 + 688582088681764130469*u^6 - 
        25698037955845496067927*u^4 + 444470604942195922015755*u^2 - 2654155080367803900605025,
    u^28 - 4190*u^26 + 7631083*u^24 - 7953124300*u^22 + 5258554468937*u^20 - 2313326757869890*u^18 + 691451285514065259*u^16 - 141062107217586416040*u^14 + 19477099336547993586171*u^12 - 
        1781103872658227723795970*u^10 + 103764470143371018680338137*u^8 - 3607131084573924222894990540*u^6 + 66647887693999747894954784187*u^4 - 515514421669410774166185623070*u^2 + 
        658183121944091618062137174225,
    u^28 - 5030*u^26 + 11062483*u^24 - 14011323580*u^22 + 11334903338297*u^20 - 6144004874030170*u^18 + 2278980307315212579*u^16 - 581103493011642321480*u^14 + 101012541960287565780891*u^12 - 
        11721148039976818734548730*u^10 + 874805354519020136234930097*u^8 - 39464316038445853713270113340*u^6 + 965293690052644951685914832427*u^4 - 10251056885167335152229172745670*u^2 + 
        22496297740087585881559134267225,
    u^30 - 6215*u^28 + 17130553*u^26 - 27660223855*u^24 + 29120754272117*u^22 - 21062188449251635*u^20 + 10746912594180061629*u^18 - 3912472954846506174795*u^16 + 1016495041382905711558371*u^14 
        - 186649036097625271828470645*u^12 + 23724143583811307738887542507*u^10 - 2014327681114638603202628104845*u^8 + 107706664173932221886003619561447*u^6 - 
        3275040635073408166774303148786385*u^4 + 46223767186821792521108512535217375*u^2 - 161848299820393930940736081066149625,
    u^34 - 7409*u^32 + 24536968*u^30 - 48044061352*u^28 + 62011604202572*u^26 - 55716323980459948*u^24 + 35891263834688596824*u^22 - 16834010372865538440696*u^20 + 5784142367682972998073846*u^18
        - 1454577177258528345405792054*u^16 + 265803147697085157663921639672*u^14 - 34814117251261327600339394217048*u^12 + 3198299132462390401751355821033772*u^10 - 
        199456338312339967657105726079921868*u^8 + 8030605583842133022357136589098359720*u^6 - 192263355629320573841421425357773413000*u^4 + 2343774565101526911963134582229265892625*u^2 - 
        9828773601650947807037135802518643590625,
    u^36 - 8922*u^34 + 35942625*u^32 - 86613009776*u^30 + 139456761311028*u^28 - 158770869887812824*u^26 + 131968104321088284388*u^24 - 81555689542506113038608*u^22 + 
        37825078574164084230497454*u^20 - 13201878596465416664388944412*u^18 + 3457656060197250890830997255454*u^16 - 673914592533742850008437431909904*u^14 + 
        96348840519098806403158113274617156*u^12 - 9884079413438783153042461727511491544*u^10 + 704202993321246822210236318693162146644*u^8 - 33174165749358438162669533651865847643760*u^6 + 
        955247483973393143985725367826535240657625*u^4 - 14571916199301874811516071682256921725372250*u^2 + 83485118007548616960116261168240503676615625,
    u^38 - 10299*u^36 + 48053115*u^34 - 134591529905*u^32 + 252836914507428*u^30 - 337196546939276172*u^28 + 329719310975039022268*u^26 - 240804213684248591554932*u^24 + 
        132630810520582421871375294*u^22 - 55269305298829419954942864906*u^20 + 17388428070562644113267770115514*u^18 - 4100761780126515438464290485677166*u^16 + 
        715900171197020354056858977779880276*u^14 - 90781039646030263424963725109231697564*u^12 + 8136358902914585418605983625327773296684*u^10 - 495636357324944841996396510592087348473156*u^8 +
        19377956522391710329343230845695393006281545*u^6 - 445101064049179071492123249432148597706416275*u^4 + 5177020655347055691181765069853799767253211875*u^2 - 
        22711032246441393516231062038675228977768515625,
    u^44 - 12302*u^42 + 69239935*u^40 - 236610412148*u^38 + 549459541784707*u^36 - 919748248913270486*u^34 + 1148989069656897835213*u^32 - 1094474723973849448826480*u^30 + 
        805533314533281755701371226*u^28 - 461541928967718110253944237052*u^26 + 206514429127544387915748094513446*u^24 - 72119441118339869972121541587076920*u^22 + 
        19577196457693502603026719624834404502*u^20 - 4099121776759328236737053383626986012604*u^18 + 654170727960937096861203148250462720819850*u^16 - 
        78212503734767115379758317319774926243800176*u^14 + 6836980008003428572296900814856434321006155189*u^12 - 422028250886223501142365592098345343850710857462*u^10 + 
        17476800084974190439148752639441918166326024419531*u^8 - 448540393629268182677088044978029477583305447285620*u^6 + 6253526937210642323596984565394593401672539709730775*u^4 - 
        37013087756228993438266827460643377762894550851248750*u^2 + 36216052456609571501642100973941635690472733838765625,
    u^46 - 14031*u^44 + 90335373*u^42 - 354240358323*u^40 + 947213106563319*u^38 - 1832474477909116569*u^36 + 2656412406399120683427*u^34 - 2949330083696933261665917*u^32 + 
        2542635629725269645990850506*u^30 - 1716023204830753337160717361366*u^28 + 910300057801399334581742561189154*u^26 - 379794917031561601278650463117488094*u^24 + 
        124336205057946458110180824996594824142*u^22 - 31772020098712725043423144410922885842642*u^20 + 6284329779658963921858699025096861417340486*u^18 - 
        950723639808086517376724704211459154945758586*u^16 + 108221758508007120716431396804586924534558859813*u^14 - 9064589955315235203964631233978893112556710422123*u^12 + 
        541703810142100407507035758346162718031056350211009*u^10 - 22099490581355673902428565998394662574147261960627199*u^8 + 575519241478602744849692362953831221973866961860056395*u^6 - 
        8548391828613695055518850344595330692379013546865979525*u^4 + 57660526157018663778791066029295076251556455534269086375*u^2 - 78851361024240485411617502746826081749310666651673365625,
    u^48 - 16320*u^46 + 122969772*u^44 - 568239863280*u^42 + 1804272351857466*u^40 - 4180458832412028960*u^38 + 7327400482038443155308*u^36 - 9941553290905188829088880*u^34 + 
        10597879412161076190377899959*u^32 - 8961103027118366974327485544960*u^30 + 6043062815709362851488367382794008*u^28 - 3257537904747726258175107458551396320*u^26 + 
        1402926089030566422040476636036315061068*u^24 - 481206107617813404344149235190101938921920*u^22 + 130693492089010146644109714544139281079733624*u^20 - 
        27861214431816761323633025479939809705582649440*u^18 + 4605355440290385066382236116544429865412814118527*u^16 - 580575147464824232829796388314804916750808355110720*u^14 + 
        54588756010586412191469378287247213923692967741129916*u^12 - 3713289930628647399685191601644916637780394002370926640*u^10 + 175023963429571473882972256380825430032139261446202739226*u^8 
        - 5358105116029793696443300156039467992466432822068402230560*u^6 + 95705632190084918805694266035334522853543081441769191225500*u^4 - 
        806068626799434151187330983634170709507930057683943400222000*u^2 + 1633028894458907038375112951888851130489017543200471929315625,
    u^50 - 18513*u^48 + 158759532*u^46 - 837966978396*u^44 + 3051274900260906*u^42 - 8143365283470357498*u^40 + 16522088906396221243788*u^38 - 26091295675814223353868444*u^36 + 
        32575051076875286943465173799*u^34 - 32487926211658849885708572723367*u^32 + 26051689293305457508735490442488088*u^30 - 16856670894850965155306467591911773304*u^28 + 
        8810609240253765832820024161388607971628*u^26 - 3715825953299389208353368500342996947019724*u^24 + 1260393521354278710160860222535160130802985784*u^22 - 
        341953923857080301928265780290319130842620080472*u^20 + 73611595534806797471329647461701239963596171777247*u^18 - 12434212321276816063621495536567252503862022665489711*u^16 + 
        1623506067815872910526177067222134055453785198617466876*u^14 - 160547483860116240901557743807851625327186860833766862508*u^12 + 
        11691340160478092845439797345671290436120822979417512815946*u^10 - 602329015821336029750582751546149185747962792127316114494938*u^8 + 
        20667103189165206527160393164274650604267258326066253085134780*u^6 - 427410677849240510576873946996630547713982360585781036021167500*u^4 + 
        4381673155828631757347164831657134493953089231944341249149921625*u^2 - 12619895974634802361962873893903066819063199842760411048413165625,
    u^54 - 21275*u^52 + 210738079*u^50 - 1292063306925*u^48 + 5499015837149070*u^46 - 17271241628616207450*u^44 + 41550355320230213370570*u^42 - 78452334018807621327923550*u^40 + 
        118188927313103472012635286315*u^38 - 143676595134575485835117341314025*u^36 + 142009993743460306783202621600090621*u^34 - 114665422132971712825151450379682810375*u^32 + 
        75820638017149763033405691176413486028724*u^30 - 41075494477001392307789385170405612112128700*u^28 + 18206317158508720004337244936885961304222675900*u^26 - 
        6581509960159023613972826983386013812550619474100*u^24 + 1930603385755422673759819738271155397135403714989895*u^22 - 456263632534723800309728944156684828544762545312888125*u^20 + 
        86044979565786509915725018695058596352261404001828372905*u^18 - 12786719006810995395884180421588769048934972548455094423275*u^16 + 
        1472989848611893856300342207940966252409684156477604123702238*u^14 - 128742192678654273120274604952117342297165006643123282688440650*u^12 + 
        8296537362425691056901442812663679320402482851571124363309662682*u^10 - 379046899146325825426705676586372448991779093731089199561295841550*u^8 + 
        11604726090333594514705322139825495469458407984035183392946537366125*u^6 - 218045642929676872490390960081914526911679771799262827595041979329375*u^4 + 
        2141494099506780114603784813343744187723304687455117498409416680566875*u^2 - 7355108808988902119186519358232848256241818181827213285683215865890625,
    u^56 - 23756*u^54 + 263271754*u^52 - 1809718138524*u^50 + 8654588479722795*u^48 - 30616427016346045320*u^46 + 83173670498734791900420*u^44 - 177825812402519203544749320*u^42 + 
        304258929154298290232382241065*u^40 - 421456305354315578613475454226340*u^38 + 476384655672459005288832799220468246*u^36 - 441674837439964633985412491472800351476*u^34 + 
        336886480266062438503460670316323638236299*u^32 - 211641237160483315718545097402407936441053744*u^30 + 109456958088799724247167787526062270994924879800*u^28 - 
        46508739041808758214399428760088568117058582970800*u^26 + 16178113247995858032194132189784607044239272493681595*u^24 - 4583250540718227184585857385313945349010623553708840020*u^22 + 
        1050127047441444425294586284479770325296768657041864047830*u^20 - 192839160304412819602062844074661905185458065665856384291780*u^18 + 
        28053708050304605919770388724663858306713402532760822415245913*u^16 - 3185437480341561900997296299042091521583539525771193019162102728*u^14 + 
        276930192665518364019255539462872120890546137991816598891514121732*u^12 - 17968892277011633353266120314791443364564467175092657476842987413192*u^10 + 
        840276219724405534835226437016577634396568690720467651120023015995675*u^8 - 26917639815779741642301023023647999385630679996495296938447550925485500*u^6 + 
        545249906921862328083762949703723398083680073546765256502693262821546250*u^4 - 6037428140154643242867861598705542018422830816706882064905838538344307500*u^2 + 
        25728219609552457719128241701834592088745585092508282400464894826574640625,
    u^62 - 27215*u^60 + 347323633*u^58 - 2765177880735*u^56 + 15412738736753961*u^54 - 63992397533068590375*u^52 + 205603399848138992751225*u^50 - 524306015966808362439338775*u^48 + 
        1080033058975555004343086821845*u^46 - 1819841629029953040399344366662075*u^44 + 2530950261486588672251990695715741381*u^42 - 2923883726686799018635181514722817000715*u^40 + 
        2818081608914676159960189372672784131485133*u^38 - 2272140388631916883262629716997926110837744835*u^36 + 1534477470300346829456219195293275823057737630621*u^34 - 
        868024283531612447627856207998728622735552276577075*u^32 + 410798099636072675184900615839621960114610035169448995*u^30 - 162259427839589585099159711586810387666551456972904773325*u^28 + 
        53296096258782918443830764435596890041740570717953248773235*u^26 - 14484893202037022647818090843626727243632611879770037463281725*u^24 + 
        3236183080822856065277557789919689308913730096278296455688159483*u^22 - 589423000879603496902577886805832318806283939911799723082473977845*u^20 + 
        86600045335024979033399364698694632792586345418749303611411902999659*u^18 - 10127875310113431977967886442437625528473588355000832373420845574811205*u^16 + 
        926956859653091487349013818039115483684196420349169675763876602490245703*u^14 - 64957195990966811499627135591203363817787517517722747797434796636318677225*u^12 + 
        3385817504524706561426184201294878829747609367562115490882324668653167716375*u^10 - 126200484232340148649906209509891464221534419636192622449704863835371112625625*u^8 + 
        3180126773979703079805223327780756568624522458285413504949569370852766472039375*u^6 - 49746018840414406173654312391043271389451367132377795190909489269016665986390625*u^4 + 
        418632078385904895055921055855245103073201308869996825574014217462286427112109375*u^2 - 1412616904993906679281459423116407109828683681633361003306248304128591901181640625,
    u^64 - 30024*u^62 + 423208968*u^60 - 3725746730632*u^58 + 22990944897234576*u^56 - 105807121004215426824*u^54 + 377270528208301863954600*u^52 - 1068985860222317089179011400*u^50 + 
        2449725197222149675110213733620*u^48 - 4597637493528758211581600810965480*u^46 + 7130689081033085300050950624639924456*u^44 - 9197702744727615754211486300769990178344*u^42 + 
        9909895094200506054886216795317372812623168*u^40 - 8942829118166124286166838103329009305297979432*u^38 + 6768002867842430211404132460644370381815862521736*u^36 - 
        4295785298276558198342168260628116821905499260489064*u^34 + 2284142886314509437863978775768778552372994666328601470*u^32 - 1015070714289125097222151520657922481410805776693750910680*u^30
        + 375688572706996889378446164300677806966862359544557687710360*u^28 - 115242548839697482497580108780134476550731397171898762837862040*u^26 + 
        29113830593661396071461373763515115223877426659974767101660990608*u^24 - 6008661287269674351804740434393913842408922020550033025578922471192*u^22 + 
        1002804731492415182671585857493653523136103069125965596269450887014264*u^20 - 133605354901582330049242847424268177688400598097612172316796081621080536*u^18 + 
        13979714910219817410127978777895047295783054125650525790875998487668982948*u^16 - 1124857807353069393693104073415634345941477978450549825615586166011367695352*u^14 + 
        67703123317568112251516063892190183771749115850626860260380529821894788948600*u^12 - 2936150551001941037559684748596462909308509299224269597153131508421878972899000*u^10 + 
        87038149732462891342782066295389581650379145306829256718481483437029890668660000*u^8 - 1630424699150344792280977241430716587389796478277320576262240880092800411179395000*u^6 + 
        17006927933000478746226136998544397609001281917106727359290932034571847734742375000*u^4 - 78132591060053028880450165318129766906586047413353080642205983567481596866846875000*u^2 + 
        65710224456753436257747042686700719053150881984670123431210012796875229244853515625,
    u^66 - 33777*u^64 + 537461520*u^62 - 5361059277136*u^60 + 37633101855261912*u^58 - 197865924301865785752*u^56 + 809775472507560879875952*u^54 - 2646719927352970724501434800*u^52 + 
        7034171277925309045650096308220*u^50 - 15399365784796438764116640586838140*u^48 + 28033332951422189218421817870228087696*u^46 - 42727038724537882621002574967702004284112*u^44 + 
        54789164303299435135608978672228353421872680*u^42 - 59300521396552253428826310898945343579860949736*u^40 + 54276505098450456953133247293877848882577469980272*u^38 - 
        42038839812218213521817648893814167280321911034865072*u^36 + 27541569418411097383595409674833598511074428469325752742*u^34 - 
        15239564867778705482053387930762082202995458591432591353990*u^32 + 7103572466415478661343149878129112957308922100185428612647600*u^30 - 
        2778928354158200490865313557479900149661718913177149983924862320*u^28 + 907826525667326463856744054748117630240160141609468178892068340328*u^26 - 
        246070222864536052648123991495464280700379955266289879771400403880616*u^24 + 54893080274589516737478026817597457005419440202469956050857791359600080*u^22 - 
        9975996092919297475172619631187219271122003103541843192887640953212918928*u^20 + 1458236152986546721541668778371375357112392981218799145459603177488860498876*u^18 - 
        168701991718861677513464103377342848290362220507983982811102375736681062187196*u^16 + 15130106387132765283583770314703340718189179313522390814958748171183684862584496*u^14 - 
        1023798189175953626169463584206224265581423594460657854198981834393933010112562800*u^12 + 50388794332817690221195812757437432442150868021208996465392774949783018355784127000*u^10 - 
        1713207196882194300448538293595369526936373340014933065712061861455807896894894375000*u^8 + 37257761358936740529196797609667748602421256903463210087576127177004112279943712210000*u^6 - 
        457345735956757050122637456697238997261215583577554208288529904116959701789431390250000*u^4 + 2500165862307093471768011961476084891103939126670033355073584471833099191351790925390625*u^2
        - 2543463134337368374377363338892676567554481453828849428330432561831591107343991494140625,
    u^72 - 37484*u^70 + 663513934*u^68 - 7381994027836*u^66 + 57963776289182177*u^64 - 341961927915243452128*u^62 + 1575710083438696916350800*u^60 - 5820435428764967931744092640*u^58 + 
        17554721236594747006353563229108*u^56 - 43813376732351657266365709112194192*u^54 + 91392824061494495533377395571444471176*u^52 - 160524263929763687195915367295081255397584*u^50 + 
        238725554787367809233644604053124830154893924*u^48 - 301817508321076860872570097542008641668645096096*u^46 + 325316062745966817597340447830821386019382894613552*u^44 - 
        299476470266188390736133873364096816005126620322388128*u^42 + 235669808387297653715774441039641320150240519059755875630*u^40 - 
        158547624057821398289283785158318858268515161155288370444360*u^38 + 91121868478299190871795915700626399149293558589437898509185748*u^36 - 
        44673832112606129489504522052531802449001294628254346440749533352*u^34 + 18641199121384868525784910895896625260381838677381917751417764651678*u^32 - 
        6600086907008100784227785024813049507436702407041939223086883014897952*u^30 + 1974948609174272953439885593563402557164917638344560552473889987680097072*u^28 - 
        496967796127094062489029978824324967111030197474252552555045158665063571488*u^26 + 104518587133395502914693743149430972141297665006277373509220498879156983406276*u^24 - 
        18233510266623133245647097023154257415290649850249571894463044960712314089576464*u^22 + 2614153078054028845365996502600067688096778368991440940119677921378395640860926600*u^20 - 
        304512604421109435426565094378061367793644360263438875188229307223838042622767722320*u^18 + 28411404103569490792856468100160250895547650493755065474403057591026424116325450848724*u^16 - 
        2085116810785365568051987420212852715849573957800236369616495770984066126099491461338976*u^14 + 
        117574127598613854036903858413505596762159069911397593505423808602657410910204959581483600*u^12 - 
        4935738542832382176929182571839968378754052457306713698057577506564202916005908606846044000*u^10 + 
        147589227109244986084118331887728820945809617059013382219165804439292027248745255710766785625*u^8 - 
        2942168353091520832080980454741601912537892927980807568320074960223087250820406951000771747500*u^6 + 
        35032419167911754433599483074810847341380202244847239098375060693644222782204270312153679468750*u^4 - 
        199823301397685632954721397436260674874359083122408886140489957673313643122932007483178548437500*u^2 + 
        259565529578689706214464607923132510823245797473272833303318966397026810076206007300277041015625
]

